Reinforcement Learning in Non-Stationary Environments

Reinforcement learning (RL) methods learn optimal decisions in the presence of a stationary environment. However, the stationary assumption on the environment is very restrictive. In many real world problems like traffic signal control, robotic applications, one often encounters situations with non-stationary environments and in these scenarios, RL methods yield sub-optimal decisions. In this paper, we thus consider the problem of developing RL methods that obtain optimal decisions in a non-stationary environment. The goal of this problem is to maximize the long-term discounted reward achieved when the underlying model of the environment changes over time. To achieve this, we first adapt a change point algorithm to detect change in the statistics of the environment and then develop an RL algorithm that maximizes the long-run reward accrued. We illustrate that our change point method detects change in the model of the environment effectively and thus facilitates the RL algorithm in maximizing the long-run reward. We further validate the effectiveness of the proposed solution on non-stationary random Markov decision processes, a sensor energy management problem and a traffic signal control problem.

==> abs-ai2019.tex <==
\begin{abstract}
Reinforcement learning (RL) methods learn optimal decisions in the presence of a stationary environment. However, the stationary assumption on the environment is very restrictive. In many real world problems like traffic signal control, robotic applications, etc., one often encounters situations with non-stationary environments and in these scenarios, RL methods yield sub-optimal decisions. In this paper, we thus consider the problem of developing RL methods that obtain optimal decisions in a non-stationary environment. The goal of this problem is to maximize the long-term discounted reward accrued when the underlying model of the environment changes over time. To achieve this, we first adapt a change point algorithm to detect change in the statistics of  the environment and then develop an RL algorithm that maximizes the long-run reward accrued. We illustrate that our change point method detects change in the model of the environment effectively and thus facilitates the RL algorithm in maximizing the long-run reward. We further validate the effectiveness of the proposed solution on non-stationary
random Markov decision processes, a sensor energy management problem and a traffic signal control problem.
% \\\emph{\hspace*{0.3cm}Note to Practitioners}--- This paper is motivated by the problem of efficient energy management in a energy harvesting (EH) sensor node. 
% The sensor is typically powered using a energy buffer that stores energy harvested from the ambient environment. 
% The amount of energy harvested from the environment is stochastic in nature, and is usually modeled as a random quantity whose values are sampled from a probability distribution. 
% The goal of the controller here is to enable the sensor node to work perpetually and efficiently. This it needs to do by intelligently deciding on the amount of energy to be utilized from the energy buffer in order to transmit the data stored in the data buffer to a central server. 
% This induces a tradeoff between the delay in the transmitted data and the amount of energy drawn from the buffer.
% A natural problem arises when the modelling assumption on the energy harvested from a probability distribution changes, as it happens in case of for e.g., solar energy. A sensor can harvest more solar energy around noon, but energy collection dips during evening time and is zero during night. Under such change in the statistics of the energy harvesting process, how does one enable the sensor node to achieve efficient operation? 
% Our paper suggests a general RL method that can help in intelligent automation of physical systems where there is a need for optimal management of resources under changing system conditions. Using this method an automated system controller can know when the operating conditions have changed and accordingly adjust its behaviour to improve the system's efficiency and performance. Preliminary simulations suggest that this approach is feasible and effective. Our method depends only on the data collected from the system and assumes sufficient data could be obtained on a fixed system condition in order to detect change in the system condition effectively. 
% For a complex system, this means that lot of data has to be collected and hence scalability of our method is an issue.
% In future research, we will address the issue of scalability.
\end{abstract}

